Rethinking the Role of Token Retrieval in Multi-Vector Retrieval

Multi-vector retrieval models such as ColBERT [Khattab and Zaharia, 2020] allow token-level interactions between queries and documents, and hence achieve state of the art on many information retrieval benchmarks. However, their non-linear scoring function cannot be scaled to millions of documents, necessitating a three-stage process for inference: retrieving initial candidates via token retrieval, accessing all token vectors, and scoring the initial candidate documents. The non-linear scoring function is applied over all token vectors of each candidate document, making the inference process complicated and slow. In this paper, we aim to simplify the multi-vector retrieval by rethinking the role of token retrieval. We present XTR, ConteXtualized Token Retriever, which introduces a simple, yet novel, objective function that encourages the model to retrieve the most important document tokens first. The improvement to token retrieval allows XTR to rank candidates only using the retrieved tokens rather than all tokens in the document, and enables a newly designed scoring stage that is two-to-three orders of magnitude cheaper than that of ColBERT. On the popular BEIR benchmark, XTR advances the state-of-the-art by 2.8 nDCG@10 without any distillation. Detailed analysis confirms our decision to revisit the token retrieval stage, as XTR demonstrates much better recall of the token retrieval stage compared to ColBERT.

==> figures/all-examples_bak.tex <==
\begin{table*}[ht]
\centering
\footnotesize
\begin{tabular}{ccp{11cm}}

\toprule 
% \multicolumn{3}{c}{Query: what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19?} \\ \midrule

\multicolumn{3}{l}{\textbf{T5-ColBERT} token retrieval for ``\textit{how \textcolor{Blue}{\textbf{much}} do jockeys have to weigh}?''} \\
\midrule
Rank & Token & Context of Token \\
\midrule
0	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does a skid steer weigh? quick answer. skid steers can weigh between 2,050 and 10,520 pounds, depending on the manufacturer and the model.  \\
1	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} should an english bulldog weigh? how much should an english bulldog weigh? an adult male english bulldog should weigh between 53 and 55 pounds, and an adult female should weigh between 49 and 51 pounds.  \\
2	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does a club car golf cart weigh? quick answer. a club car golf cart generally weighs between 500 and 600 pounds (or 225 to 275 kg).  \\
3	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does a baby calf weigh? quick answer. the average weight of a calf at birth is 63.6 pounds for females. male calves weigh about 5 percent more at birth.  \\
4	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} do bench press bars usually weigh? bart loews, trains strength every spare minute of the day. standard bars are 45 pounds (20 kg). shorter bars can weight between 20 and 40 pounds.  \\
5	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does a grizzly bear weigh? quick answer. adult female grizzly bears can weigh from 200 to 450 pounds, while the adult male of the species weighs anywhere from 300 to 850 pounds. the largest \\
6	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does a basset hound weigh? confidence votes 3.7k. the average weight for a male basset hound is between 50 and 65 pounds (23-29kg) and for a female is between 45 and 60 pounds \\
7	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} do sumo wrestlers weigh, on average? answer wiki. in the top division, makuuchi (42 wrestlers), i'd say the minimum weight you'll see is 300 lbs, or close \\
8	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does a husky weigh? a: the average weight range for a male husky is between 45 and 60 pounds. the average weight for a female husky is between 35 and 50 pounds. siberian \\

\midrule 
\\ \midrule

\multicolumn{3}{l}{\textbf{\ours} token retrieval for ``\textit{how \textcolor{Blue}{\textbf{much}} do jockeys have to weigh}?''} \\ 
\midrule
Rank & Token & Context of Token \\ 
\midrule
0	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does a jockey have to weigh? there is no specific weight but you wouldn't want to be very heavy but you should be well under 200 id say 150 is a good weight but lower is good. \\
1	& \textcolor{Blue}{\textbf{more}}	& weight control among jockeys to make weight in anything but high-class stakes races, jockeys had to keep their weight to no \textcolor{Blue}{\textbf{more}} than 114 lbs. riders competing in ordinary weekday events needed to whittle themselves down another 5 lbs or so, while those in the lowest echelons of the sport could not weight much more than 100.\\
2	& \textcolor{Blue}{\textbf{pounds}}	& """what it takes to be jockey"" by frank lovato jr" jockeys should weigh approximately 110 pounds and apprentices (rookies) 105 \textcolor{Blue}{\textbf{pounds}} or less. if you are already much heavier then that, for your health, please reconsider the idea of wanting to be a jockey.\\
3	& \textcolor{Blue}{\textbf{l}}	& jockey the weight of a jockey usually ranges from 108 to 118  \textcolor{Blue}{\textbf{l}}b (49 to 54 kg). despite their light weight, they must be able to control a horse that is moving at 40 mph (64 km/h) and weighs 1,200 lb (540 kg).\\
4	& \textcolor{Blue}{\textbf{much}}	& need to weight to be a jump jockey or exercise. dont quote me exactly but i think jump jockeys have to weigh about 9 stone max.  \textcolor{Blue}{\textbf{much}} do i need to weight to be a jump jockey or exercise. i'm just looking for the average but most say the max (or average max, as there isn't a maximum weight. \\
5	& \textcolor{Blue}{\textbf{pounds}}	& """what it takes to be jockey"" by frank lovato jr" jockeys should weigh approximately 110 pounds and apprentices (rookies) 105 \textcolor{Blue}{\textbf{pounds}} or less. if you are already much heavier then that, for your health, please reconsider the idea of wanting to be a jockey. \\
6	& \textcolor{Blue}{\textbf{much}}	& thread: how much do i need to weight to be a jump jockey or exercise rid re: how \textcolor{Blue}{\textbf{much}} do i need to weight to be a jump jockey or exercise. dont quote me exactly but i think jump jockeys have to weigh about 9 stone max. \\
7	& \textcolor{Blue}{\textbf{from}}	& jockey the kentucky derby, for example, has a weight limit of 126 lb (57 kg) including the jockey's equipment. the weight of a jockey usually ranges \textcolor{Blue}{\textbf{from}} 108 to 118 lb (49 to 54 kg). \\
8	& \textcolor{Blue}{\textbf{from}}	& jockey the weight of a jockey usually ranges \textcolor{Blue}{\textbf{from}} 108 to 118 lb (49 to 54 kg).  \\
% 9	& \textcolor{Blue}{\textbf{much}}	& how \textcolor{Blue}{\textbf{much}} does the average pit bull weigh? quick answer. the weight range for an average american pit bull terrier varies greatly and can be between 25 and 85 pounds. male pit bulls usually weigh between 35 and 65 pounds. \\

\bottomrule
\end{tabular}
\caption{Token retrieval example from MS MARCO for the token \textit{``much''} in the query \textit{``how much do jockeys have to weight''}. T5-ColBERT retrieve \textit{``much''} from off-topic passages; XTR retrieves sematically related tokens from passages about the weight of jockeys. } 
\end{table*}


%============ New Example ===========
\begin{table*}%[h]
\centering
\footnotesize
\begin{tabular}{ccp{11cm}}

\toprule 
% \multicolumn{3}{c}{Query: what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19?} \\ \midrule

\multicolumn{3}{l}{\textbf{T5-ColBERT} token retrieval for ``\textit{cost of hiv/aids  \textcolor{Blue}{\textbf{yearly}} treatment}''} \\
\midrule
Rank & Token & Context of Token \\
\midrule
0	& \textcolor{Blue}{\textbf{yearly}}	& for as much as you'd spend on lunch one day, you get unlimited access to a plethora of movies and tv shows, often award-winning ones that are produced and only available on netflix. so  \textcolor{Blue}{\textbf{yearly}}, it would cost \$95.88 for basic, \$119.88 for standard, or \$143.88 for premium. \\
1	& \textcolor{Blue}{\textbf{yearly}}	& autism costs average \$17,000  \textcolor{Blue}{\textbf{yearly}} for each child autism costs average \$17,000 yearly for each child. \\
2	& \textcolor{Blue}{\textbf{yearly}}	& the mean  \textcolor{Blue}{\textbf{yearly}} costs (expressed in 1991 prices) of epilepsy-related health care including antiepileptic drug treatment was us \$1,594 the year before starting gvg therapy \\
3	& \textcolor{Blue}{\textbf{yearly}}	& all together how much does it cost on a dog per year? plan on going to the vet for wellness checkups once or twice a year at a cost of at least \$150-300  \textcolor{Blue}{\textbf{yearly}}. annual blood work can add about \$100-200. \\
4	& \textcolor{Blue}{\textbf{yearly}}	& if you live in a more expensive smoking state such as hawaii, the  \textcolor{Blue}{\textbf{yearly}} cost is closer to \$3,500. \\
5	& \textcolor{Blue}{\textbf{yearly}}	& the cost of diabetes the approximate  \textcolor{Blue}{\textbf{yearly}} total for pumping is \$2500. the approximate yearly total for for mdi is \$900. \\
6	& \textcolor{Blue}{\textbf{yearly}}	& on a dog per year? routine veterinary care is a huge part of keeping your dog healthy. plan on going to the vet for wellness checkups once or twice a year at a cost of at least \$150-300  \textcolor{Blue}{\textbf{yearly}}.  \\
7	& \textcolor{Blue}{\textbf{yearly}}	& on a dog per year? routine veterinary care is a huge part of keeping your dog healthy. plan on going to the vet for wellness checkups once or twice a year at a cost of at least \$150-300  \textcolor{Blue}{\textbf{yearly}}.  \\
8	& \textcolor{Blue}{\textbf{yearly}}	& average cost for outpatient stroke rehabilitation services and medications the first year post inpatient rehabilitation discharge was \$17,081. the corresponding average  \textcolor{Blue}{\textbf{yearly}} cost of medication was \$5,392, while the average cost of yearly rehabilitation service utilization was \$11,689. \\
% 9	& \textcolor{Blue}{\textbf{yearly}}	& the cost of diabetes the approximate  \textcolor{Blue}{\textbf{yearly}} total for pumping is \$2500. the approximate yearly total for for mdi is \$900. based on this rough calculation, if doctor visits average \$1000 a year, diabetes has cost me \$23,000 to \$50,000 \\

\\ \midrule

\multicolumn{3}{l}{\textbf{\ours} token retrieval for ``\textit{cost of hiv/aids  \textcolor{Blue}{\textbf{yearly}} treatment''}} \\ 
\midrule
Rank & Token & Context of Token \\ \midrule

0	& \textcolor{Blue}{\textbf{year}}	& 1 the average cost of hiv treatment per \textcolor{Blue}{\textbf{year}} is \$14,000 to \$25,000. 2 for instance, a monthly hiv treatment regimen can range anywhere from \$2,000 to \$6,000. \\
1	& \textcolor{Blue}{\textbf{year}}	& 1 on average, the lifetime cost of care for a person living with hiv could total up to hundreds of thousands of dollars. 2 the average cost of hiv treatment per \textcolor{Blue}{\textbf{year}} is \$14,000 to \$25,000. 3 for instance, a monthly hiv treatment regimen can range anywhere from \$2,000 to \$6,000.\\
2	& \textcolor{Blue}{\textbf{year}}	& hiv treatment is costly, especially for the sickest patients the average total cost of hiv care was \$19,912 per patient per \textcolor{Blue}{\textbf{year}}. costs were highest for patients with advanced disease. the cost for providing care to each patient who died was \$44,000. \\
3	& \textcolor{Blue}{\textbf{year}}	& hiv treatment is costly, especially for the sickest patients the average total cost of hiv care was \$19,912 per patient per \textcolor{Blue}{\textbf{year}}. costs were highest for patients with advanced disease. \\
4	& \textcolor{Blue}{\textbf{year}}	& the average total cost of hiv care was \$19,912 per patient per \textcolor{Blue}{\textbf{year}}. costs were highest for patients with advanced disease. \\
5	& \textcolor{Blue}{\textbf{yearly}}	& autism costs average \$17,000 yearly for each child autism costs average \$17,000  \textcolor{Blue}{\textbf{yearly}} for each child.\\
6	& \textcolor{Blue}{\textbf{yearly}}	& average yearly dog vet costs some controversy over vaccinations should prompt you to conduct further research into which shots may be most beneficial and how long the effects may last. on average, expect to pay between \$150 and \$300 for  \textcolor{Blue}{\textbf{yearly}} vet bills, including shots.dental work is necessary to keep teeth healthy and prevent other types of infection and disease.\\
7	& \textcolor{Blue}{\textbf{year}}	& york city-based advocacy group for people with hiv. on september 14, 1989, members of act up protested at the new york stock exchange over the burroughs wellcome's setting a price of \$10,000 usd per \textcolor{Blue}{\textbf{year}} for azt, which was the only effective treatment for hiv discovered. \\
8	& \textcolor{Blue}{\textbf{year}}	& certain forms of a treatment for leukemia can cost each patient as much as \$138,000 per \textcolor{Blue}{\textbf{year}}. that is not uncommon for drugs to get rid of cancer and keep it away. \\
% 9	& \textcolor{Blue}{\textbf{year}}	& can you afford your hiv treatment? the average cost of hiv treatment is \$14,000 to \$20,000 a \textcolor{Blue}{\textbf{year}}, says michael kolber, md, a professor of medicine and director of the comprehensive aids program and adult hiv services at university of miami miller school of medicine in florida.\\
\bottomrule
\end{tabular}
\caption{Token retrieval example from MS MARCO for the token \textit{``yearly''} in the query \textit{``cost of hiv/aids yearly treatment''}. T5-ColBERT retrieve \textit{``yearly''} from off-topic passages; XTR retrieves \textit{``yearly''} and its lexcial variants \textit{``year''} with the top 5 passages having the relevant context about HIV treatment costs. } 
\end{table*}

%============ New Example ===========
\begin{table*}%[h]
\centering
\footnotesize
\begin{tabular}{ccp{11cm}}

\toprule 
% \multicolumn{3}{c}{Query: what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19?} \\ \midrule

\multicolumn{3}{l}{\textbf{T5-ColBERT} token retrieval for ``\textit{
\textcolor{Blue}{\textbf{why}} did franklin d roosevelt launch a new programs during his first hundred days in office}?''} \\
\midrule
Rank & Token & Context of Token \\
\midrule
0	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} did the u.s. support the mujahideen against the soviet union in afghanistan? \\
1	& \textcolor{Blue}{\textbf{why}}	& in nicaragua's civil war that began in 1979, \textcolor{Blue}{\textbf{why}} did the united states support the contras against the sandinistas \\
2	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} did king george iii and parliament tax the colonists between 1764 and 1774? what were these taxes? \\
3	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} does the writer select the three video games mentioned in paragraphs 5;6;7 and 8 to be included in the olympics \\
4	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} did the farmers of the constitution stipulate that federal judges be appointed, rather than elected, and serve for life? \\
5	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} is it necessary to keep making rubp in the cycle?  \\
6	& \textcolor{Blue}{\textbf{why}}	& a quick guide to mission san jose for visitors and students no one knows exactly \textcolor{Blue}{\textbf{why}} san jose mission was built here \\
7	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} the department of justice wants to force its 28,000 employees to confront unconscious racial biases. \\
8	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} do presidents rely so heavily on staff in the white house office and the executive office of the presidency? \\
9	& \textcolor{Blue}{\textbf{why}}	& aim assist in games... why? okay, so i already know \textcolor{Blue}{\textbf{why}} we have aim assist in games.  \\
\midrule 
\\ \midrule

\multicolumn{3}{l}{\textbf{\ours} token retrieval for ``\textit{
\textcolor{Blue}{\textbf{why}} did franklin d roosevelt launch a new programs during his first hundred days in office}?''} \\ 
\midrule
Rank & Token & Context of Token \\  \midrule
0	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} did franklin roosevelt launch new deal programs during his first hundred days in office? \\
1	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} did the u.s. support the mujahideen against the soviet union in afghanistan? \\
2	& \textcolor{Blue}{\textbf{because}}	& fdr packed supreme court with judges who were sympathetic to his new deal \textcolor{Blue}{\textbf{because}} his new deal allowed congress to begin spending government money and he needed people who suppported his idea of keynesian economics or the tax and spend policy which allowed the government to spend beyond its means.\\
3	& \textcolor{Blue}{\textbf{because}}	& number of reasons to oppose it many northerners where against it and he wanted to maintain the union and he didn't want to anger the border states. but he decided in favor of the emancipation proclamation \textcolor{Blue}{\textbf{because}} he wanted to weaken the south. \\
4	& \textcolor{Blue}{\textbf{why}}	&  part from fahrenheit 9/11 by michael moore where u see \textcolor{Blue}{\textbf{why}} the congress obviously passed the patriot act. conspiracy theorists often point out that the patriot act is taking away the liberties of the us citizens, and that it is only one of the first steps towards fascism.but\\
5	& \textcolor{Blue}{\textbf{because}}	& new deal farm laws. \textcolor{Blue}{\textbf{because}} president roosevelt's advisors believed that the economic depression had been caused by an economic slowdown in farming, much of the new deal was intended to help farmers. \\
6	& \textcolor{Blue}{\textbf{why}}	& moving america forward 2012 democratic national platform government is more accountable when it is transparent. that is \textcolor{Blue}{\textbf{why}} president obama signed the memorandum on transparency and open government on his first full day in office \\
7	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} was franklin d. roosevelt elected president 4 times? roosevelt was elected president mainly as a result of the great depression, in 1932 and in 1936\\
8	& \textcolor{Blue}{\textbf{why}}	& \textcolor{Blue}{\textbf{why}} did franklin d. roosevelt run for a third term in 1940? because the us was at war and changing presidents during this time may have upset the trust of the american public. edit\\
9	& \textcolor{Blue}{\textbf{to}}	&'s encyclopedia (ages 8-11) the new deal was a group of u.s. government programs of the 1930s. president franklin d. roosevelt started the programs \textcolor{Blue}{\textbf{to}} help the country recover from the economic problems of the great depression.\\

\bottomrule
\end{tabular}
\caption{Token retrieval example from MS MARCO for the token \textit{``why''} in the query \textit{``why did franklin d roosevelt launch a new program during his first hundred days in office?''}. T5-ColBERT retrieve \textit{``why''} from off-topic passages; XTR retrieves sematically related tokens such as \textit{``because''} and \textit{``to''} from passages related to the query. } 
\end{table*}


%============ New Example ===========
% \begin{table*}%[h]
% \centering
% \footnotesize
% \begin{tabular}{ccp{11cm}}

% \toprule 
% % \multicolumn{3}{c}{Query: what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19?} \\ \midrule

% \multicolumn{3}{l}{\textbf{T5-ColBERT} token retrieval for ``\textit{\textcolor{Blue}{\textbf{cost}} for child cineplex}?''} \\
% \midrule
% Rank & Token & Context of Token \\
% \midrule
% 0	& \textcolor{Blue}{\textbf{cost}}	& faqs this price includes having you arrive a few minutes early to greet each other, and includes a few minutes after class for using the changing rooms and stretching. \textcolor{Blue}{\textbf{cost}} for 6-7 people is \$40 per person, for 5 it is \$45 per person for 4 or fewer it is \$200 flat fee. \\
% 1	& \textcolor{Blue}{\textbf{cost}}	& the \textcolor{Blue}{\textbf{cost}} of the individual ticket, including the contribution for the guide, is 12,00 euros(approximately \$15.50 usd) [from january 1, 2013: the cost of the individual ticket is 13,00 euros \\
% 2	& \textcolor{Blue}{\textbf{costs}}	& in general, the minimum \textcolor{Blue}{\textbf{costs}} is \$99 for up to 3 players. every additional player is \$33. the minimum cost is higher during peak hours. please also be aware that room escape is a live event, so once the booking is confirmed, refunds, reschedules, and cancellations are not accepted. \\
% 3	& \textcolor{Blue}{\textbf{costs}}	& if you are a us subscriber it \textcolor{Blue}{\textbf{costs}} \$19.95 which includes postage for one month rolling subscription. if you are a uk subscriber it costs \$29.95  \\
% 4	& \textcolor{Blue}{\textbf{cost}}	&the minimum \textcolor{Blue}{\textbf{cost}} is higher during peak hours. please also be aware that room escape is a live event, so once the booking is confirmed, refunds, reschedules, and cancellations are not accepted. \\
% 5	& \textcolor{Blue}{\textbf{cost}}	& dog vaccination cost dog vaccination cost. 1 the average cost for dog vaccinations ranges from \$20 to \$150 in the first year, and from \$10 to \$100 per year afterward. the \textcolor{Blue}{\textbf{cost}} varies based on which vaccinations are given and whether they are done at a veterinarian's office or a low-cost vaccination clinic run by a local government or humane organization. \\
% 6	& \textcolor{Blue}{\textbf{cost}}	& duplication of 5 \\
% 7	& \textcolor{Blue}{\textbf{cost}}	& duplication of 5 \\
% 8	& \textcolor{Blue}{\textbf{cost}}	& \textcolor{Blue}{\textbf{cost}} of fare. the cost of tickets to use the channel tunnel varies depending on what time of day you go, the day, and the size of your vehicle.   \\
% % 9	& \textcolor{Blue}{\textbf{cost}}	& the average cost for dog vaccinations ranges from \$20 to \$150 in the first year, and from \$10 to \$100 per year afterward. the \textcolor{Blue}{\textbf{cost}} varies based on which vaccinations are given and whether they are done at a veterinarian's office or a low-cost vaccination clinic run by a local government or humane organization. \\
% \midrule 
% \\ \midrule

% \multicolumn{3}{l}{\textbf{\ours} token retrieval for ``\textit{\textcolor{Blue}{\textbf{cost}} for child cineplex}?''} \\ 
% \midrule
% Rank & Token & Context of Token \\ 
% \midrule
% 0	& \textcolor{Blue}{\textbf{for}}	& at regal, on a tuesday, i can see a movie with popcorn for \$7. at cinemark, with a pass, i can see a 3d movie with popcorn (anytime) \textcolor{Blue}{\textbf{for}} \$9.75.</s>\\
% 1	& \textcolor{Blue}{\textbf{about}}	& this place was a nice surprise. indoor air-conditioned amusement park for kids and adults. brought our 2.5 year-old here, and he had a great time. he rode all the rides he wanted for \textcolor{Blue}{\textbf{about}} \$18 (junior ticket).</s>\\
% 2	& \textcolor{Blue}{\textbf{cost}}	& as united artists and edwards theaters) are showing almost free summer movies for kids june through august in 2017. showtimes are 10:00 a.m. every tuesday and wednesday and \textcolor{Blue}{\textbf{cost}} \$1. \\
% 3	& \textcolor{Blue}{\textbf{cost}}	& your family vacation just got a little more expensive. last year, walt disney world announced that ticket prices for those 10 and up at the magic kingdom in orlando now exceed \$100. single-day tickets \textcolor{Blue}{\textbf{cost}} \$105 per day for ages 10 and up or \$99 for kids 3-9.</s>\\
% 4	& \textcolor{Blue}{\textbf{is}}	& memorial day weekend activities all active and retired military personnel will receive one free adventure pass with valid id and will save up to 30\% off per person (ticket \textcolor{Blue}{\textbf{is}} \$23.95 + tax for an adult or child) for immediate family members, and will receive 20\% off food and merchandise. .</s>\\
% 5	& \textcolor{Blue}{\textbf{is}}	& it's actually called disneyland and is located in anaheim, not los angeles. the cost for a single day, single park ticket \textcolor{Blue}{\textbf{is}} currently \$90.53 for an adult and \$84.14 for a child. \\
% 6	& \textcolor{Blue}{\textbf{at}}	& cup for \$3.75 from cinemark when you buy a fountain or frozen beverage. 2 10\% bonus on any ticket purchase. 3 6\% bonus on any box office purchase. prices cut up to 32\% on six movie tickets to classic films marked \textcolor{Blue}{\textbf{at}} \$30.</s>\\
% 7	& \textcolor{Blue}{\textbf{are}}	& disneyland ticket discounts, deals \& coupons 1 adult (10 years and older) 4-day disneyland park hopper plus 1-day legoland california tickets \textcolor{Blue}{\textbf{are}} \$352, plus a \$2 convenience fee, which is \$31 less than the gate price of the same set of tickets. </s>\\
% 8	& \textcolor{Blue}{\textbf{cost}}	& disney parks has raised the price of admission to disney world in 2015. single-day tickets to the magic kingdom now \textcolor{Blue}{\textbf{cost}} \$105 for adults, while one-day admission to epcot, animal kingdom and disney's hollywood studios cost \$97 for adults.</s>\\
% % 9	& \textcolor{Blue}{\textbf{is}}	&ney world raises admission prices for second time in a year after spending \$1.5 billion on hi-tech tracking wristbands better start saving: the price of a one-day ticket to walt disney world's magic kingdom \textcolor{Blue}{\textbf{is}} now \$99. \\
% \bottomrule
% \end{tabular}
% \caption{Example.} 
% \end{table*}

%============ New Example ===========
\begin{table*}%[h]
\centering
\footnotesize
\begin{tabular}{ccp{11cm}}

\toprule 
% \multicolumn{3}{c}{Query: what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19?} \\ \midrule

\multicolumn{3}{l}{\textbf{T5-ColBERT} token retrieval for ``\textit{another \textcolor{Blue}{\textbf{word}} for density}''} \\
\midrule
Rank & Token & Context of Token \\
\midrule

0	& \textcolor{Blue}{\textbf{word}}	& another \textcolor{Blue}{\textbf{word}} for interpretation. another word for interpretation word list. below are a number of words whose meaning is similar to interpretation. 1 elucidation. 2 explanation. 3 exposition. \\
1	& \textcolor{Blue}{\textbf{word}}	& another \textcolor{Blue}{\textbf{word}} for attitude word list. below are a number of words whose meaning is similar to attitude. 1 pose. 2 position. 3 posture. \\
2	& \textcolor{Blue}{\textbf{word}}	& what is another word for an operating system? os. another \textcolor{Blue}{\textbf{word}} for operating. it's gui(graphical user interface) os. different version of windows operating and microsoft office problem. modern operating systems can also be called graphical user interfaces (gui).  \\
3	& \textcolor{Blue}{\textbf{word}}	& what is another \textcolor{Blue}{\textbf{word}} for an operating system? os. another word for operating. it's gui(graphical user interface) os. different version of windows operating and microsoft office problem.  \\
4	& \textcolor{Blue}{\textbf{word}}	& another \textcolor{Blue}{\textbf{word}} for density density synonyms: noun the quality, condition, or degree of being thick: compactness, solidity, thickness.  \\
5	& \textcolor{Blue}{\textbf{word}}	& another \textcolor{Blue}{\textbf{word}} for curve. another word for curve word list. below are a number of words whose meaning is similar to curve. 1 bend. 2 curvature. 3 flexure.\\
6	& \textcolor{Blue}{\textbf{word}}	& another \textcolor{Blue}{\textbf{word}} for constitution another word for constitution. 3 to 50 characters max. the act of founding or establishing: creation, establishment, foundation, institution, organization, origination, start-up. \\
7	& \textcolor{Blue}{\textbf{word}}	& what is another \textcolor{Blue}{\textbf{word}} for stress relief? answers.comÂ® is making the world better one answer at a time. another word for stress relief is to de-stress.  \\
8	& \textcolor{Blue}{\textbf{word}}	& another word for cancellate another word for cancer body another word for cancer borealis another \textcolor{Blue}{\textbf{word}} for cancer cell another word for cancer drug another word for cancer irroratus other word for cancer irroratus cancer irroratus  \\
% 9	& \textcolor{Blue}{\textbf{word}}	&f-wordâ one last nail in the coffin of the 'fornication under consent of the king' origin comes from the word 'fornication' itself. though many reasonably conclude fornication is the old-time \textcolor{Blue}{\textbf{word}} for having sex, the term specifically excludes the physical union of man and wife. \\ \midrule 
\\ \midrule

\multicolumn{3}{l}{\textbf{\ours} token retrieval for ``\textit{another \textcolor{Blue}{\textbf{word}} for density}?''} \\ 
\midrule
Rank & Token & Context of Token \\ 
\midrule
0	& \textcolor{Blue}{\textbf{word}}	& another \textcolor{Blue}{\textbf{word}} for density density synonyms: noun the quality, condition, or degree of being thick: compactness, solidity, thickness. see thick \\
1	& \textcolor{Blue}{\textbf{word}}	& density synonyms and density antonyms. top synonym for density (another \textcolor{Blue}{\textbf{word}} for density) is compactness. \\
2	& \textcolor{Blue}{\textbf{words}}	& what are some alternative \textcolor{Blue}{\textbf{words}} for density? synonyms for density. this thesaurus page is about all possible synonyms, equivalent, same meaning and similar words for the term density. \\
3	& \textcolor{Blue}{\textbf{words}}	& what are some alternative words for density? synonyms for density. this thesaurus page is about all possible synonyms, equivalent, same meaning and similar \textcolor{Blue}{\textbf{words}} for the term density. princeton's wordnet (3.00 / 3 votes) rate these synonyms: density, denseness (noun) \\
4	& \textcolor{Blue}{\textbf{synonym}}	& density synonyms and density antonyms. top \textcolor{Blue}{\textbf{synonym}} for density (another word for density) is compactness. \\
5	& \textcolor{Blue}{\textbf{synonym}}	& visual synonyms of density princeton's wordnet(4.00 / 2 votes)rate these \textcolor{Blue}{\textbf{synonym}}s: 1 density, denseness(noun) the amount per unit size. synonyms: 2 concentration, density, denseness, tightness, compactness(noun) \\
6	& \textcolor{Blue}{\textbf{synonym}}	& synonyms for density in free thesaurus. antonyms for density. 20 \textcolor{Blue}{\textbf{synonym}}s for density: tightness, closeness, thickness, compactness, impenetrability, denseness, crowdedness, mass, body, bulk, consistency, solidity.... what are synonyms for density? \\
7	& \textcolor{Blue}{\textbf{synonym}}	& princeton's wordnet(4.00 / 2 votes)rate these \textcolor{Blue}{\textbf{synonym}}s: 1 density, denseness(noun) the amount per unit size. 2 concentration, density, denseness, tightness, compactness(noun) the spatial property of being crowded together. \\
8	& \textcolor{Blue}{\textbf{synonym}} & this thesaurus page is about all possible synonyms, equivalent, same meaning and similar words for the term density. princeton's wordnet (3.00 / 3 votes) rate these \textcolor{Blue}{\textbf{synonym}}s: density, denseness (noun) \\
% 9	& \textcolor{Blue}{\textbf{synonym}}	& \textcolor{Blue}{\textbf{synonym}}s for density: cohesion, compactness, denseness, solidity, thickness, breadth, bulk, caliber, diameter, expanse, width, firmness, rigidity, security, snugness, stiffness \\
 \bottomrule
\end{tabular}
\caption{Token retrieval example from MS MARCO for the token \textit{``word''} in the query \textit{``another word for density''}. T5-ColBERT retrieve \textit{``word''} from off-topic passages; XTR retrieves sematically related tokens such as \textit{``words''} and \textit{``synonym''} from passages related to definition and synonyms of density. } \zhuyun{5 examples and correct context label (1,2, 5, 50, 100). In caption add how many lexical overlap we have in top 100. } \end{table*}



%============ New Example ===========
\begin{table*}%[h]
\centering
\footnotesize
\begin{tabular}{ccp{11cm}}

\toprule 
% \multicolumn{3}{c}{Query: what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19?} \\ \midrule

\multicolumn{3}{l}{\textbf{T5-ColBERT} token retrieval for ``\textit{how has \textcolor{Blue}{\textbf{co}}vid-19 affected canada}?''} \\
\midrule
Rank & Token & Context of Token \\
\midrule
0	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19's impact on genetics at one medical center in new york. \\
1	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 and schools closure: implications for school nurses. \\
2	& \textcolor{Blue}{\textbf{co}}	& does \textcolor{Blue}{\textbf{co}}vid-19 affect male fertility? \\
3	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 and lockdown: delayed effects on health \\
4	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19's impact on genetics at one medical center in new york \\
5	& \textcolor{Blue}{\textbf{co}}	& impact of \textcolor{Blue}{\textbf{co}}vid-19 outbreak on acute low back pain \\
6	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 affects healthy pediatricians more than pediatric patients \\
7	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 presents high risk to older persons \\
8	& \textcolor{Blue}{\textbf{co}}	& impact of \textcolor{Blue}{\textbf{co}}vid-19 on veterinary care \\
9	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 strikes the vulnerable. \\


 \midrule 
\\ \midrule

\multicolumn{3}{l}{\textbf{\ours} token retrieval for ``\textit{how has \textcolor{Blue}{\textbf{co}}vid-19 affected canada}?''} \\ 
\midrule
Rank & Token & Context of Token \\ 
\midrule
0	& \textcolor{Blue}{\textbf{co}}	& canada’s \textcolor{Blue}{\textbf{co}}vid-19 response: navigating national and global solidarity \\
1	& \textcolor{Blue}{\textbf{co}}	& community health workers reveal \textcolor{Blue}{\textbf{co}}vid-19 disaster in brazil \\
2	& \textcolor{Blue}{\textbf{co}}	& understanding heterogeneity to inform the public health response to \textcolor{Blue}{\textbf{co}}vid-19 in canada \\
3	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 in brazil \\
4	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 in brazil \\
5	& \textcolor{Blue}{\textbf{co}}	& impact of \textcolor{Blue}{\textbf{co}}vid-19 on tuberculosis control in china \\
6	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 in africa: between hope and reality \\
7	& \textcolor{Blue}{\textbf{co}}	& australia and the \textcolor{Blue}{\textbf{co}}vid-19 crisis \\
8	& \textcolor{Blue}{\textbf{co}}	& nicaragua's surprising response to \textcolor{Blue}{\textbf{co}}vid-19 \\
9	& \textcolor{Blue}{\textbf{co}}	& \textcolor{Blue}{\textbf{co}}vid-19 in africa: no room for complacency \\


\bottomrule
\end{tabular}
\caption{Token retrieval example from TREC-COVID for the token \textit{``co''} (in \textit{``covid''}) in the query \textit{``how has covid-19 affected canada''}. T5-ColBERT retrieves \textit{``co''} from off-topic passages; XTR retrieves  \textit{``co''}  from passages related tp covid-19's impacts on various locations. }  
\end{table*}

%============ New Example ===========
\begin{table*}%[h]
\centering
\footnotesize
\begin{tabular}{ccp{11cm}}

\toprule 
% \multicolumn{3}{c}{Query: what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19?} \\ \midrule

\multicolumn{3}{l}{\textbf{T5-ColBERT} token retrieval for ``\textit{what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19??''}} \\ \midrule
Rank & Token & Context of Token \\
\midrule
0	& \textcolor{Blue}{\textbf{best}}	&. bubble continuous positive airway pressure (bcpap) can offer effective and affordable non-invasive respiratory support. objective to determine the \textcolor{Blue}{\textbf{best}} physical components of bubble cpap circuits for respiratory support of children in low-resource settings.  \\
1	& \textcolor{Blue}{\textbf{best}}	& paritaprevir, ritonavir, entecavir and chloroquine derivatives are the \textcolor{Blue}{\textbf{best}} drugs to inhibit multi targets of coronavirus infection including natural compounds corosolic acid, baicalin and glycyrrhizic acid with minimal inhibitory concentrations.  \\
2	& \textcolor{Blue}{\textbf{best}}	& paritaprevir, ritonavir, entecavir and chloroquine derivatives are the \textcolor{Blue}{\textbf{best}} drugs to inhibit multi targets of coronavirus infection including natural compounds corosolic acid, baicalin and glycyrrhizic acid with minimal inhibitory concentrations. \\
3	& \textcolor{Blue}{\textbf{best}}	&l4 (rpl4) and tyrosine 3-monooxygenase tryptophan 5-monooxygenase activation protein zeta polypeptide (ywhaz) are the \textcolor{Blue}{\textbf{best}} reference genes to use in the study of host cell response to h5n1 aiv infection.  \\
4	& \textcolor{Blue}{\textbf{best}}	&  the \textcolor{Blue}{\textbf{best}} form of vitamin d for use in the treatment of respiratory diseases is calcitriol because it is the active metabolite of vitamin d3 and modulates inflammatory cytokine expression.  \\
5	& \textcolor{Blue}{\textbf{best}}	&   although a variety of interfaces are available, the oronasal mask is the \textcolor{Blue}{\textbf{best}} initial interface in terms of leak prevention and patient comfort.  \\
6	& \textcolor{Blue}{\textbf{best}}	&  oxygen concentrators are usually the \textcolor{Blue}{\textbf{best}} source of oxygen. as yet, there is no affordable and accurate oxygen blender. \\
7	& \textcolor{Blue}{\textbf{best}}	& paritaprevir, ritonavir, entecavir and chloroquine derivatives are the \textcolor{Blue}{\textbf{best}} drugs to inhibit multi targets of coronavirus infection including natural compounds corosolic acid, baicalin and glycyrrhizic acid with minimal inhibitory concentrations \\
8	& \textcolor{Blue}{\textbf{best}}	&the \textcolor{Blue}{\textbf{best}} parameter for diagnosing septic arthritis was synovial lactate (auc = 0.864, sensitivity = 74.5\%, specificity = 87.2\%) \\
9	& \textcolor{Blue}{\textbf{best}}	& peb (85\%) and everolimus-eluting stents (68\%) had the greatest probabilities for being the \textcolor{Blue}{\textbf{best}} treatment option. furthermore, peb were the best treatment in terms of late luminal loss (85\%) and binary restenosis (85\%).  \\


 \midrule 
\\ \midrule

\multicolumn{3}{l}{\textbf{\ours} token retrieval for ``\textit{what are the \textcolor{Blue}{\textbf{best}} masks for preventing infection by covid-19??''}} \\ 
\midrule
Rank & Token & Context of Token \\ 
\midrule
0	& \textcolor{Blue}{\textbf{best}}	& there was a significant difference in efficiency between the best and worst masks. the \textcolor{Blue}{\textbf{best}} masks contained more fabric, were softer and were pleated, while the worst were stiffer, smaller and not pleated. \\
1	& \textcolor{Blue}{\textbf{best}}	& transocular transmission of laiv occured in most participants suggesting the necessity of eye protection. an n95 respirator provided the \textcolor{Blue}{\textbf{best}} guard further enhanced by eye protection. \\
2	& \textcolor{Blue}{\textbf{best}}	& there was a significant difference in efficiency between the \textcolor{Blue}{\textbf{best}} and worst masks. the best masks contained more fabric, were softer and were pleated, while the worst were stiffer, smaller and not pleated. \\
3	& \textcolor{Blue}{\textbf{best}}	& choosing the \textcolor{Blue}{\textbf{best}} supraglottic airway for ophthalmic general anaesthesia: a manikin study general anaesthesia is sometimes favoured over regional anaesthesia in ophthalmic surgery. \\
4	& \textcolor{Blue}{\textbf{better}}	&  we found no direct high quality evidence on whether n95 respirators are \textcolor{Blue}{\textbf{better}} than surgical masks for hcws protection from sars-cov-2. \\
5	& \textcolor{Blue}{\textbf{better}}	&  we found no direct high quality evidence on whether n95 respirators are \textcolor{Blue}{\textbf{better}} than surgical masks for hcws protection from sars-cov-2. \\
6	& \textcolor{Blue}{\textbf{better}}	&  interpretation we found no direct high quality evidence on whether n95 respirators are \textcolor{Blue}{\textbf{better}} than surgical masks for hcws protection from sars-cov-2. however, low quality evidence suggests that n95 respirators protect hcws from clinical respiratory infections. \\
7	& \textcolor{Blue}{\textbf{best}}	&  it is unclear which type of ppe protects best, what is the \textcolor{Blue}{\textbf{best}} way to remove ppe, and how to make sure hcws use ppe as instructed. \\
8	& \textcolor{Blue}{\textbf{good}}	& covid-19: are face masks a \textcolor{Blue}{\textbf{good}} long term strategy? \\
9	& \textcolor{Blue}{\textbf{better}}	&  although cloth masks generally perform poorer than the medical grade masks, they may be \textcolor{Blue}{\textbf{better}} than no masks at all.  \\


\bottomrule
\end{tabular}
\caption{Token retrieval example from TREC-COVID for the token \textit{``best''}  in the query \textit{``what are the best masks for preventing infection by covid-19?''}. T5-ColBERT retrieves \textit{``best''} from off-topic passages; XTR retrieves  \textit{``best''}, \textit{``better''}, and \textit{``good''}from passages related to masks. }  
\end{table*}

==> figures/latency.tex <==
\begin{figure}[t!]
    \centering
    \resizebox{0.5\columnwidth}{!}{%
        \includegraphics[width=.3\textwidth]{figures/msmarco-token.png}
    }
    \caption{
    Refinement latency comparison of T5-ColBERT and XTR.
    Each refinement latency is measured by changing the token retrieval top $k^\prime$.
    We report MRR@10 on the MS MARCO development set.\jinhyuk{placeholder image used}
    \jinhyuk{this figure might look bit empty, make it inline?}}
    \label{fig:latency}
    % \vspace{-.3cm}
\end{figure}


==> figures/lexical-retrieval.tex <==
\begin{figure}[t!]
    \centering
    \resizebox{1.0\columnwidth}{!}{%
        \includegraphics[width=.30\textwidth]{figures/lex-msmarco.pdf}\hfill
        \includegraphics[width=.30\textwidth]{figures/lex-trec-covid.pdf}\hfill
        \includegraphics[width=.30\textwidth]{figures/lex-arguana.pdf}
    }
    \caption{
    Lexical token retrieval performances of T5-ColBERT and XTR.
    We plot the probability of each retrieved document token at rank $k$ being lexically equal to its query token.
    % (e.g., \textit{what are the chances of retrieving a document token \textbf{hello} for a query token \textbf{hello}?}).
    % For each dataset, we sample 1,000 test query tokens and compute the probability with their top-1000 document tokens.
    % \jinhyuk{qualitative samples of which tokens were retrieved would be great (apdx)}
    % \zhuyun{Good to show in qualitative samples that T5-ColBERT retrieve irrelevant exact match tokens that are in completely different context.}
    % \jinhyuk{lower height}
    }
    \label{fig:lex-retrieval}
    \vspace{-.2cm}
\end{figure}



==> tables/lotte.tex <==
\begin{table}
\small
\centering
\resizebox{1.00\linewidth}{!}{%
\begin{tabular}{lccccccccccccc}
\toprule
    & \multicolumn{6}{c}{\textbf{LoTTE Search}} && \multicolumn{6}{c}{\textbf{LoTTE Forum}} \\ % && \multicolumn{3}{c}{\textbf{Open-domain QA}} \\
    \cmidrule{2-7} \cmidrule{9-14} % \cmidrule{16-18}
    & Writing & Rec. & Sci. & Tech. & Life. & Pooled && Writing & Rec. & Sci. & Tech. & Life. & Pooled \\ % && NQ & TQA & SQD \\
    \midrule
    % \multicolumn{18}{c}{\textit{In-domain Retrieval}} \\
    % \midrule
    % DPR & & & & & & & & & & & & & & & 66.8 & 70.8 & - \\
    % DensePhrases & & & & & & & & & & & & & & &  69.9 & 75.0 & -\\
    % \midrule
    % \multicolumn{18}{c}{\textit{Zero-shot Retrieval}} \\
    % \midrule
    BM25 & 60.3 & 56.5 & 32.7 & 41.8 & 63.8 & 48.3 && 64.0 & 55.4 & 37.1 & 39.4 & 60.6 & 47.2 \\
    ColBERT & 74.7 & 68.5 & 53.6 & 61.9 & 80.2 & 67.3 && 71.0 & 65.6 & 41.8 & 48.5 & 73.0 & 58.2 \\
    GTR$_\text{base}$ & 74.1 & 65.7 & 49.8 & 58.1 & 82.0 & 65.0 && 69.2 & 62.0 & 33.7 & 47.6 & 72.2 & 54.9 \\
    \rowcolor{lightgray} \textbf{XTR$_\text{base}$} & 77.0 & 69.4 & 54.9 & 63.2 & 82.1 & 69.0 && 73.9 & 68.7 & 42.2 & 51.9 & 74.4 & 60.1 \\
    \midrule
    ANCE$^\vardiamondsuit$ & 74.4 & 64.7 & 53.6 & 59.6 & 82.3 & 66.4 && 68.8 & 63.8 & 36.5 & 46.8 & 73.1 & 55.7 \\
    % Splade$_\text{v2}$$^{\clubsuit\vardiamondsuit}$ & 77.1 & 69.0 & 55.4 & 62.4 & 82.3 & 68.9 && 73.0 & 67.1 & 43.7 & 50.8 & 74.0 & 60.1 \\
    RocketQA$_\text{v2}$$^{\clubsuit\vardiamondsuit}$ & 78.0 & 72.1 &  55.3 &  63.4 &  82.1 & 69.8 &&  71.5 &  65.7 &  38.0 &  47.3 & 73.7 & 57.7 \\
    ColBERT$_\text{v2}$$^{\clubsuit\vardiamondsuit}$ & 80.1 & 72.3 & 56.7 & 66.1 & 84.7 & 71.6 && 76.3 & 70.8 & 46.1 & 53.6 &76.9 & 63.4 \\
    \midrule
    GTR$_\text{xxl}$ & \textbf{83.9} & 78.0 & 60.0 & 69.5 & 87.4 & 76.0 && 79.5 & 73.5 & 43.1 & 62.6 & 81.9 & 66.9\\
    \rowcolor{lightgray} \textbf{XTR$_\text{xxl}$} & {83.3} & \textbf{79.3} &  \textbf{60.8} & \textbf{73.7} & \textbf{89.1} & \textbf{77.3} && \textbf{83.4} & \textbf{78.4} & \textbf{51.8} & \textbf{64.5} & \textbf{83.9} & \textbf{71.2} \\
\bottomrule
\end{tabular}
}

\begin{tablenotes}
      \scriptsize
      \item $\clubsuit$: cross-encoder distillation \quad $\vardiamondsuit$: model-based hard negatives
\end{tablenotes}
\caption{Zero-shot top-5 retrieval accuracy (success@5) on LoTTE datasets.
While \ours{}$_\text{base}$ remains competitive with the distillation-based models, scaling \ours greatly advances the state-of-the-art.
% \jinhyuk{results pending}
% \jinhyuk{add average}
% \jinhyuk{GTR}
% \jinhyuk{move openQA results to the last columns}
% \jinhyuk{numbers from where}
}\label{tab:lotte}
\end{table}
